Maximum Likelihood Time Synchronization for Zero-padded OFDM

Existing Orthogonal Frequency-Division Multiplexing (OFDM) variants based on cyclic prefix (CP) allow for efficient time synchronization, but suffer from lower power efficiency compared to zero-padded (ZP)-OFDM. Because of its power efficiency, ZP-OFDM is considered as an appealing solution for the emerging low-power wireless systems. However, in the absence of CP, time synchronization in ZP-OFDM is a very challenging task. In this paper, the non-data-aided (NDA) maximum-likelihood (ML) time synchronization for ZP-OFDM is analytically derived. We show that the optimal NDA-ML synchronization algorithm offers a high lock-in probability and can be efficiently implemented using Monte Carlo sampling (MCS) technique in combination with golden-section search. To obtain the optimal NDA-ML time synchronization algorithm, we first derive a closed-form expression for the joint probability density function (PDF) of the received ZP-OFDM samples in frequency-selective fading channels. The derived expression is valid for doubly-selective fading channels with mobile users as well. The performance of the proposed synchronization algorithm is evaluated under various practical settings through simulation experiments. It is shown that the proposed optimal NDA-ML synchronization algorithm and its MCS implementation substantially outperforms existing algorithms in terms of lock-in probability.

==> Wgroup-Teaching-Preamble.tex <==
% Greek lowercase letters, sans serif font - by Guido
%
%% =========== Euler ==========
%\DeclareMathAlphabet{\matheur}{U}{eur}{m}{n}
%\SetMathAlphabet{\matheur}{bold}{U}{eur}{b}{n}
%\DeclareRobustCommand{\msf}[1]{%
%  \ifcat\noexpand#1\relax\msfgreek{#1}\else\matheur{#1}\fi%for math sans serif (Euler)
%}
%% =========================
%
% ==== Computer Modern Sans Serif ====
%\DeclareMathAlphabet{\mathsfbr}{OT1}{cmss}{m}{n}%for math sans serif (cmss)
%\SetMathAlphabet{\mathsfbr}{bold}{OT1}{cmss}{bx}{n}%for math sans serif (cmss)
%\DeclareRobustCommand{\msf}[1]{%
%  \ifcat\noexpand#1\relax\msfgreek{#1}\else\mathsfbr{#1}\fi%for math sans serif (cmss)
%}
% =========================

% ==== Computer Modern Bright ====
% Part 1: This is necessary to fix a bug in the .fd file of the font!!!
\DeclareFontFamily{OT1}{cmbr}{\hyphenchar\font45 }
\DeclareFontShape{OT1}{cmbr}{m}{n}{%
  <-9>cmbr8
  <9-10>cmbr9
  <10-17>cmbr10
  <17->cmbr17
}{}
\DeclareFontShape{OT1}{cmbr}{m}{sl}{%
  <-9>cmbrsl8
  <9-10>cmbrsl9
  <10-17>cmbrsl10
  <17->cmbrsl17
}{}
\DeclareFontShape{OT1}{cmbr}{m}{it}{%
  <->ssub*cmbr/m/sl
}{}
\DeclareFontShape{OT1}{cmbr}{b}{n}{%
  <->ssub*cmbr/bx/n
}{}
\DeclareFontShape{OT1}{cmbr}{bx}{n}{%
  <->cmbrbx10
}{}
% Part 2
\DeclareMathAlphabet{\mathsfbr}{OT1}{cmbr}{m}{n}%for math sans serif bright (cmbr)
\SetMathAlphabet{\mathsfbr}{bold}{OT1}{cmbr}{b}{n}%for math sans serif bright (cmbr)
\DeclareRobustCommand{\msf}[1]{%
  \ifcat\noexpand#1\relax\msfgreek{#1}\else\mathsfbr{#1}\fi%for math sans serif bright (cmbr)
}
% =========================

\makeatletter
\newcommand{\msfgreek}[1]{\csname s\expandafter\@gobble\string#1\endcsname}
\makeatother

% Sans serif greek
\DeclareSymbolFont{sfletters}{U}{eur}{m}{n}\SetSymbolFont{sfletters}{bold}{U}{eur}{b}{n}%for Euler Greek
%\DeclareSymbolFont{sfletters}{FMS}{futm}{m}{n}\SetSymbolFont{sfletters}{bold}{FMS}{futm}{b}{n}%for Euler Greek

\DeclareMathSymbol{\sGamma}{\mathord}{sfletters}{0}
\DeclareMathSymbol{\sDelta}{\mathord}{sfletters}{1}
\DeclareMathSymbol{\sTheta}{\mathord}{sfletters}{2}
\DeclareMathSymbol{\sLambda}{\mathord}{sfletters}{3}
\DeclareMathSymbol{\sXi}{\mathord}{sfletters}{4}
\DeclareMathSymbol{\sPi}{\mathord}{sfletters}{5}
\DeclareMathSymbol{\sSigma}{\mathord}{sfletters}{6}
\DeclareMathSymbol{\sUpsilon}{\mathord}{sfletters}{7}
\DeclareMathSymbol{\sPhi}{\mathord}{sfletters}{8}
\DeclareMathSymbol{\sPsi}{\mathord}{sfletters}{9}
\DeclareMathSymbol{\sOmega}{\mathord}{sfletters}{10}
\DeclareMathSymbol{\salpha}{\mathord}{sfletters}{"0B}
\DeclareMathSymbol{\sbeta}{\mathord}{sfletters}{"0C}
\DeclareMathSymbol{\sgamma}{\mathord}{sfletters}{"0D}
\DeclareMathSymbol{\sdelta}{\mathord}{sfletters}{"0E}
\DeclareMathSymbol{\sepsilon}{\mathord}{sfletters}{"0F}
\DeclareMathSymbol{\szeta}{\mathord}{sfletters}{"10}
\DeclareMathSymbol{\seta}{\mathord}{sfletters}{"11}
\DeclareMathSymbol{\stheta}{\mathord}{sfletters}{"12}
\DeclareMathSymbol{\siota}{\mathord}{sfletters}{"13}
\DeclareMathSymbol{\skappa}{\mathord}{sfletters}{"14}
\DeclareMathSymbol{\slambda}{\mathord}{sfletters}{"15}
\DeclareMathSymbol{\smu}{\mathord}{sfletters}{"16}
\DeclareMathSymbol{\snu}{\mathord}{sfletters}{"17}
\DeclareMathSymbol{\sxi}{\mathord}{sfletters}{"18}
\DeclareMathSymbol{\spi}{\mathord}{sfletters}{"19}
\DeclareMathSymbol{\srho}{\mathord}{sfletters}{"1A}
\DeclareMathSymbol{\ssigma}{\mathord}{sfletters}{"1B}
\DeclareMathSymbol{\stau}{\mathord}{sfletters}{"1C}
\DeclareMathSymbol{\supsilon}{\mathord}{sfletters}{"1D}
\DeclareMathSymbol{\sphi}{\mathord}{sfletters}{"1E}
\DeclareMathSymbol{\schi}{\mathord}{sfletters}{"1F}
\DeclareMathSymbol{\spsi}{\mathord}{sfletters}{"20}
\DeclareMathSymbol{\somega}{\mathord}{sfletters}{"21}
\DeclareMathSymbol{\svarepsilon}{\mathord}{sfletters}{"22}
\DeclareMathSymbol{\svartheta}{\mathord}{sfletters}{"23}
\DeclareMathSymbol{\svarpi}{\mathord}{sfletters}{"24}
\DeclareMathSymbol{\svarrho}{\mathord}{sfletters}{"25}
\DeclareMathSymbol{\svarsigma}{\mathord}{sfletters}{"26}
\DeclareMathSymbol{\svarphi}{\mathord}{sfletters}{"27}

\DeclareRobustCommand{\mcal}[1]{%
  \ifcat\noexpand#1\relax\mathnormal{#1}\else\cal{#1}\fi
}
%-------------------------
% Math symbol
%-------------------------
\newcommand{\rv}[1]{\MakeLowercase{\msf{#1}}}  
\newcommand{\RV}[1]{\boldsymbol{\MakeLowercase{\msf{#1}}}}
\newcommand{\RM}[1]{\boldsymbol{\MakeUppercase{\msf{#1}}}}
\newcommand{\RS}[1]{\MakeUppercase{\msf{#1}}}

\newcommand{\V}[1]{\boldsymbol{\MakeLowercase{#1}}}
\newcommand{\M}[1]{\boldsymbol{\MakeUppercase{#1}}}
\newcommand{\Set}[1]{\MakeUppercase{\mcal{#1}}}

